Plateau Phenomenon in Gradient Descent Training of ReLU networks: Explanation, Quantification and Avoidance

The ability of neural networks to provide `best in class' approximation across a wide range of applications is well-documented. Nevertheless, the powerful expressivity of neural networks comes to naught if one is unable to effectively train (choose) the parameters defining the network. In general, neural networks are trained by gradient descent type optimization methods, or a stochastic variant thereof. In practice, such methods result in the loss function decreases rapidly at the beginning of training but then, after a relatively small number of steps, significantly slow down. The loss may even appear to stagnate over the period of a large number of epochs, only to then suddenly start to decrease fast again for no apparent reason. This so-called plateau phenomenon manifests itself in many learning tasks. The present work aims to identify and quantify the root causes of plateau phenomenon. No assumptions are made on the number of neurons relative to the number of training data, and our results hold for both the lazy and adaptive regimes. The main findings are: plateaux correspond to periods during which activation patterns remain constant, where activation pattern refers to the number of data points that activate a given neuron; quantification of convergence of the gradient flow dynamics; and, characterization of stationary points in terms solutions of local least squares regression lines over subsets of the training data. Based on these conclusions, we propose a new iterative training method, the Active Neuron Least Squares (ANLS), characterised by the explicit adjustment of the activation pattern at each step, which is designed to enable a quick exit from a plateau. Illustrative numerical examples are included throughout.

==> Submitted Version as of 07132020/abstract.tex <==
\begin{abstract}
  The ability of neural networks to provide ‘best in class’ approximation across
  a wide range of applications is well-documented.  Nevertheless, the powerful
  expressivity of neural networks comes to naught if one is unable to effectively
  train (choose) the parameters defining the network. In general, neural networks
  are trained by gradient descent type optimization methods, or a stochastic
  variant thereof.  In practice, such methods result in the loss function
  decreases rapidly at the beginning of training but then, after a relatively
  small number of steps, significantly slow down. The loss may even appear to
  stagnate over the period of a large number of epochs, only to then suddenly
  start to decrease fast again for no apparent reason. This so-called plateau
  phenomenon manifests itself in many learning tasks.
  
  The present work aims to identify and quantify the root causes of plateau
  phenomenon. No assumptions are made on the number of neurons relative to the
  number of training data, and our results hold for both the lazy and adaptive
  regimes. The main findings are: plateaux correspond to periods during which
  activation patterns remain constant, where activation pattern refers to the
  number of data points that activate a given neuron; quantification of
  convergence of the gradient flow dynamics; and, characterization of stationary
  points in terms solutions of local least squares regression lines over subsets
  of the training data. Based on these conclusions, we propose a new iterative
  training method, the Active Neuron Least Squares (ANLS), characterised by the  
  explicit adjustment of the activation pattern at each step, which is designed
  to enable a quick exit from a plateau.  Illustrative numerical examples are
  included throughout.
\end{abstract}

==> Submitted Version as of 07132020/conclusion.tex <==
\section{Conclusion} \label{sec:conclusion}
In this paper, we identified and quantified the root causes of plateau phenomenon
in gradient descent training of ReLU networks. 
We did not make any assumptions on the number of neurons relative to the number of training data.
By analyzing the gradient flow dynamics of univariate two-layer ReLU networks,
we showed that plateaux correspond to periods during which activation patterns remain constant, 
quantified convergence of the gradient flow dynamics,
and characterized stationary points in terms solutions of local least squares regression lines over subsets of the training data. 
Lastly, based on these conclusions, we proposed a new iterative training method, the active neuron least squares (ANLS) that is designed to quickly exit from a plateau
Numerical examples were provided to justify our theoretical findings and demonstrate the performance of ANLS.

==> Submitted Version as of 07132020/gradflow.tex <==
\section{Gradient Flow Analysis} \label{sec:GDflow}
The contribution to the error associated with the datum $(x_k,y_k)$ is measured by
$\text{loss}_{x_k}(t) = f(x_k;\bm{\theta}(t)) - y_k$,
and the corresponding residual vector is given by
\begin{align*}
\text{Loss}(t) = (\text{loss}_{x_1}(t), \cdots, \text{loss}_{x_m}(t))^T \in \mathbb{R}^m,
\end{align*}
so that $\mathcal{L}(t) = \frac{1}{2}\|\text{Loss}(t)\|_2^2$.
The equations governing the evolution of the knot $b_j$ and the coefficient $c_j$ in \eqref{def:grad-flow} are given by
\begin{equation} \label{def:bias-gradflow}
\begin{split}
\dot{b}_j(t) &= - \nabla_{b_j} \mathcal{L}(\bm{\theta}(t)) = c_j(t)\sum_{k=1}^m \text{loss}_{x_k}(t) \phi'(x_k - b_j(t)), \\
\dot{c}_j(t) &= - \nabla_{c_j} \mathcal{L}(\bm{\theta}(t)) = -\sum_{k=1}^m \text{loss}_{x_i}(t) \phi(x_k - b_j(t)), 
\end{split}
\end{equation}
subject to $b_j(0) = b_j^{(0)}$ and $c_j(0) = c_j^{(0)}$, $j=1,\cdots,n$. 
Here, $\phi'$ denotes the (left-continuous) Heaviside function
$\phi'(x) = \mathbb{I}_{x > 0}(x)$.

The discontinuity of the Heaviside function means that 
neither the Peano existence theorem nor the Picard–Lindel\"of theorem \cite{Teschl_12ODEs}
guarantee the existence of the solution to the system of ODEs \eqref{def:bias-gradflow}.
%A simple example illustrates the nonexistence of the classical solution.
%Suppose $n=m = 1$ and we train only the bias by fixing the coefficient 1.
%Then, the gradient-flow dynamics \eqref{def:bias-gradflow} reads
%\begin{align*}
%\dot{b}(t) = \begin{cases}
%-b(t) -(x_1-y_1) & \text{if } b(t) < x_1 \\
%0 & \text{if } b(t) \ge x_1
%\end{cases}.
%\end{align*}
Instead, since the right-hand side of the ODEs \eqref{def:bias-gradflow} is measurable and locally essentially bounded,
it follows from \cite{Filippov_13differential,Bressan_98Discontinuous}
that for any initial point $\bm{\theta}^{(0)}$, 
there exists a Filippov solution of \eqref{def:bias-gradflow}
with initial condition $\bm{\theta}(0) = \bm{\theta}^{(0)}$.
% we introduce a generalized notion of solution in the sense of Filippov \cite{Filippov_13differential,Bressan_98Discontinuous}.
A Filippov solution of \eqref{def:bias-gradflow}
is an absolutely continuous vector-valued function that satisfies the differential inclusion \cite{Aubin_12DiffInclusion} defined by the Filippov set-valued map.



Examining \eqref{def:bias-gradflow} shows a training point $x_k$ activates the neuron with bias $b_j$  if and only if $\phi(x_k - b_j)$ is non-zero, or equally well, $x_k > b_j$.
The set of all neurons activated by $x_k$ is given by 
\begin{equation*}
	A_k = \{ b_j | b_j < x_k \},
\end{equation*}
and the number of neurons activated by $x_k$ is $|A_k|$,
the cardinality of the set $A_k$.
%Equation \eqref{def:bias-gradflow} may be expressed in the following form using this notation:
%\begin{equation*} 
%\begin{split}
%\dot{b}_j(t) &= - \nabla_{b_j} \mathcal{L}(\bm{\theta}(t)) = c_j(t)\sum_{x \in A_j(t)} \text{loss}_{x}(t), \\
%\dot{c}_j(t) &= - \nabla_{c_j} \mathcal{L}(\bm{\theta}(t)) = -\sum_{x \in A_j(t)} \text{loss}_{x}(t)(x - b_j(t)).
%\end{split}
%\end{equation*}


The location of the $j$-th bias relative to the training points $\{x_k\}$
has a crucial impact on the flow.
For instance, in the trivial case where the initial values of the biases $\{b_j^{(0)}\}$ are chosen so that $\min_j b_j^{(0)} > \max_k x_k$, then the right hand of \eqref{def:bias-gradflow} vanishes identically meaning that 
$b_j(t) = b_j^{(0)}$ for all $t \ge 0$.
We seek to quantify this
by partitioning the training points into disjoint sets $U_l(t)$
at each time $t$, which consist of the training points $x_k$ that activate exactly
$l$ neurons, as follows:
\begin{equation} \label{def:U-set}
U_l(t) = \{x_k | |A_k| = l\}, \qquad l=0,1,\cdots,n.
\end{equation} 
The cardinality of $U_l(t)$ is denoted by $u_l(t) = |U_l(t)|$.
As a consequence, $\{U_l(t)\}_{l=0}^n$ is a partition of the training points $\{x_j\}_{j=1}^m$ and $\sum_{l=0}^n u_l(t) = m$.
In Figure~\ref{fig:set-Uk}, we illustrate $\{U_l(t)\}_{l=0}^n$ in the case $n=5$.
\begin{figure}[htbp]
	\centerline{
		\includegraphics[width=12cm]{Figures/Usets.png}
	}
	\caption{Illustration of the set $\{U_l(t)\}_{l=0}^n$ for $n=5$.
	The red dots ($\textcolor{red}{\bullet}$) show the positions of the biases $\{b_j\}$. 
	The cross marks ($\textcolor[rgb]{0.4392, 0.1882, 0.6275}{\text{\ding{54}}}$) show the positions of the training points $\{x_k\}_{k=1}^{m}$ for $m=10$.
	The set $U_l(t)$ consists of the training points which lie 
	between the $l$-th and ($l+1$)-th largest biases.
	}
	\label{fig:set-Uk}
\end{figure}


For each datum $(x,y)$, with slight abuse of notation,
we say $y \in U_l$ or $(x,y) \in U_l$ if $x \in U_l$.
The mean of the output data, and the mean and variance of the input data that correspond to the sets $\{U_l\}$ are defined respectively by
\begin{equation} \label{def:mean-variance-data}
\bar{y}_l = \frac{1}{u_l}\sum_{(x,y) \in U_l} y,
\qquad
\mu_{l} = \frac{1}{u_l}\sum_{x \in U_l} x,
\qquad
\sigma^2_{l} = \frac{1}{u_l}\sum_{x \in U_l} \left(x- \mu_{l}\right)^2.
\end{equation}

\subsection{Plateau Phenomenon}
Observe that the cardinalities $\{u_l(t)\}_{l=0}^n$ of the sets, being integer-valued, remain constant in time until
one or more of the biases $\{b_j\}$ crosses a data point,
wherein  the values of $\{u_l(t)\}$ jump to take new integer values.
The time periods, or stages, during which $\{u_l(t)\}$ remain constant play a crucial role in characterizing the evolution of the loss $\mathcal{L}(t)$ with time
as shown by the following result:

\begin{theorem} \label{thm:conti-loss-n}
	Suppose the biases and coefficients satisfy \eqref{def:bias-gradflow}, and let $[t_s,t_{s+1})$ be an interval where
	$\{u_l(t)\}$ remains constant.
	Let $\{\hat{e}^b_l, \hat{e}^c_l\}_{l=1}^n$ be vectors in $\mathbb{R}^m$
	defined as follows: for $j=1,\dots, m$,
	\begin{align*}
	[\hat{e}^b_l(t)]_j = \begin{cases}
	1 & \text{if } x_j \in U_l(t)  \\
	0 & \text{otherwise} 
	\end{cases},
	\qquad
	[\hat{e}^c_l(t)]_j 
	= \begin{cases}
	x_j - \mu_{l}  & \text{if } x_j \in U_l(t) \\
	0 & \text{otherwise} 
	\end{cases}.
	\end{align*}
	Let $V_t$ be the space spanned by $\{\hat{e}^b_l, \hat{e}^c_l\}_{l=1}^n$, $V_t^\perp$ be its orthogonal complement in $\mathbb{R}^m$,
	and $\Pi_{V}[x]$ be the orthogonal projection of $x$ onto $V$.
	Then, for $t \in [t_s,t_{s+1})$,
	\begin{align*}
	\left(\mathcal{L}(t_s) - Q_0(t_s)\right)e^{-\int_{t_s}^t \mathbf{r}_{\max}(v)dv}
	\le 
	\mathcal{L}(t) - Q_0(t_s)
	\le \left(\mathcal{L}(t_s) - Q_0(t_s)\right)e^{-\int_{t_s}^t \mathbf{r}_{\min}(v)dv}, 
	\end{align*}
	where $Q_0(t) = \frac{1}{2}\|\Pi_{V_{t}^\perp}[\text{Loss}(t)]\|^2$, and 
	$\mathbf{r}_{\min}(t)$ and $\mathbf{r}_{\max}(t)$
	are defined in Lemma~\ref{lem:def-M}.
	Furthermore, if $c_l(t) \ne 0$ for all $l$,
	$\mathbf{r}_{\min}(t)$ is strictly positive.
%	are the square of the smallest nonzero and the largest singular values of $M(t)$ defined in Lemma~\ref{lem:def-M}.
\end{theorem}
\begin{proof}
	The proof can be found in Appendix~\ref{app:thm:conti-loss-n}
\end{proof}


%\textcolor{red}{Q: Is it obvious that $Q_0(t_s)$ is monotonic decreasing with $s$?}
%\textcolor{blue}{A: The answer is no. 
%Let 
%$$
%A=V_{t_{s+1}}^\perp \cap V_{t_s}^\perp, 
%\quad 
%B =  V_{t_{s+1}}^\perp \cap V_{t_s}
%\quad 
%C = V_{t_{s+1}} \cap V_{t_s}^\perp
%\quad 
%D = V_{t_{s+1}} \cap V_{t_s}.
%$$
%Then, we see that $Q_0(t_s) = \text{proj}_{A\cup C}[\text{Loss}(t_{s})]$
%and $Q_0(t_{s+1}) = \text{proj}_{A\cup B}[\text{Loss}(t_{s+1})]$.
%Since $\text{proj}_A[\text{Loss}(t_s)] = \text{proj}_A[\text{Loss}(t_{s+1})]$,
%we have: 
%$$
%Q_0(t_s) > Q_0(t_{s+1}) \iff 
%\text{proj}_{C}[\text{Loss}(t_{s})] > \text{proj}_{B}[\text{Loss}(t_{s+1})].
%$$
%Therefore, if the component of the loss in $B$ sufficiently decays during $[t_s,t_{s+1})$, we can say $Q_0(t_s) > Q_0(t_{s+1})$.
%}

Theorem~\ref{thm:conti-loss-n} shows that for every time interval on which the activation patterns do not change, the component of the loss in the space $V_{t}$ decays exponentially at a rate determined by Lemma~\ref{lem:def-M}.
%$\{u_k, \mu_k, \sigma_k, b_k(t), c_k(t)\}$.
However, the component of the loss orthogonal to $V_{t}$ remains constant.
Throughout a time interval during which none of the biases cross a training point, the space $V_t$ does not change and the loss function decreases monotonically to the horizontal asymptote $Q_0(t_s)$.
This is precisely, the plateau phenomenon. 
The overall behavior of the loss $\mathcal{L}(t)$ consists of a number of stages during each of which $\mathcal{L}$ decreases towards a value $Q_0(t_s)$,
which depends only on the time $t_s$ at which the current stage was entered.
The value of the horizontal asymptote $Q_0(t_s)$ decreases monotonically with respect to $s$ 
(if the length of each time interval is sufficiently long).
Thus the graph of the loss with respect to the number of epochs 
takes the form of a decreasing staircase function, as shown in Figure~\ref{fig:motivation2} in section~\ref{sec:intro}.
The question of how long each interval should be 
in order for the horizontal asymptote $Q_0(t_s)$ to decrease monotonically
is addressed by the following result:

\begin{theorem} \label{thm:Q-decrease}
	Suppose the biases and coefficients satisfy \eqref{def:bias-gradflow}, and let $[t_s,t_{s+1})$ be an interval on which
	$\{u_l(t)\}$ remains constant.
	At time $t_{s+1}$, 
	suppose for some index $j$, 
	$u_l(t_s) = u_l(t_{s+1})$ for all $l$ but $j$ and $j+1$,
	and $|u_j(t_s) - u_{j}(t_{s+1})| = 1$.
	Suppose further that $t_{s+1}$ is large enough that 
	\begin{align*}
	e^{-\frac{1}{2}\int_{t_s}^{t_{s+1}} \bm{r}_{\min}(v)dv}
	< \frac{(1-|\zeta^T\psi|)|\langle \text{Loss}(t_s), \zeta \rangle|}{\|\Pi_{V_{t_s}} [\text{Loss}(t_s)] \|},
	\end{align*}
	where $\zeta \in V_{t_s}^\perp$ and $\psi \in V_{t_{s+1}}^\perp$ satisfying 
	\begin{equation*}
	\text{span}\{\zeta, \hat{e}^b_l(t_s), \hat{e}^c_l(t_s) : l=j, j+1 \}
	=\text{span}\{\psi, \hat{e}^b_l(t_{s+1}), \hat{e}^c_l(t_{s+1}) : l=j, j+1 \},
	\end{equation*}
	and $\hat{e}^b_l, \hat{e}^c_l$ are defined in Theorem~\ref{thm:conti-loss-n}.
%	are defined in Lemma~\ref{app:lem:e-vectors}.
	Then, $Q_0(t_s) > Q_0(t_{s+1})$.
\end{theorem}
\begin{proof}
	The proof can be found in Appendix~\ref{app:thm:Q-decrease}.
\end{proof}


\subsection{Convergence and Asymptotic Analysis}
Next, we show the convergence of the weight and biases to a stationary (equilibrium) point of the gradient flow dynamics \eqref{def:bias-gradflow} under the condition that the sets \eqref{def:U-set} remain trapped in a given stage, i.e., $t_{s+1} = \infty$.
We note that it is quite possible (and common in practice) for the system to remain trapped in
a given stage for all $t \ge t_s$.
For example, in the trivial case mentioned earlier in which $\min_j b_j > \max_k x_k$
the system remains in the same stage for all $t$.
See also Figures~\ref{fig:motivation-graph} and ~\ref{fig:SinPI_W10N100-BC}.

\begin{theorem} \label{thm:convergence}
	Suppose the biases and coefficients satisfy \eqref{def:bias-gradflow}, 
	$\{u_l(t)\}$ is constant for $t \in [t_s, \infty)$,
	and $c_j(t)$ does not vanish at infinity for all $j$ with $u_j(t_s) \ne 0$. 
	Then, the biases and coefficients converge
	to a stationary point
	of 	the system \eqref{def:bias-gradflow}.
%	as $t \to \infty$.
\end{theorem}
\begin{proof}
	The proof can be found in Appendix~\ref{app:thm:convergence}.
\end{proof}

%We note that Theorem~\ref{thm:convergence} admits the existence of a stationary point, which is proved by Lemma~\ref{lemma:critical}. 

As a first step towards characterizing fully trained networks, we identify necessary and sufficient conditions for the stationary (equilibrium) points of 
the system \eqref{def:bias-gradflow}.

\begin{lemma} \label{lemma:critical}
	$(\bm{b}^*,\bm{c}^*)$ is a stationary point of 
	the system \eqref{def:bias-gradflow}
	if and only if
	$(\bm{b}^*,\bm{c}^*)$
	satisfies
	\begin{equation} \label{cond:stationary}
	\begin{split}
	f(\mu_l;\bm{b}^*,\bm{c}^*) &= \bar{y}_{l}, \quad \forall l \text{ such that } u_{l} > 0, c^*_l \ne 0, \\
	\sum_{i=1}^{l} c_i^* &= 
	\frac{\frac{1}{u_l}\sum_{(x,y) \in U_l} xy - \mu_{l}\bar{y}_{l}}{\sigma^2_{l}},
	\qquad \forall l \text{ such that } u_l > 1,
	\end{split}
	\end{equation}
	where
	$\bar{y}_l, \mu_l, \sigma_l$ are defined in \eqref{def:mean-variance-data},
	and $f(x;\bm{b},\bm{c})$ is the ReLU neural network defined in \eqref{def:NN}.
	And the set of the stationary points of 
	the system \eqref{def:bias-gradflow} is nonempty.
\end{lemma}
\begin{proof}
	The proof can be found in Appendix~\ref{app:lemma:critical}.
\end{proof}


%It turns out that the stability analysis of stationary points 
%is quite challenging for the dynamics we are interested in.
A linear stability analysis reveals that 
all eigenvalues of the linearized system 
at an equilibrium point are non-positive. 
The presence of eigenvalues with vanishing real part means that 
there is a non-trivial center manifold which we shall not 
investigate in detail in the current work. 
%
%To determine stability of such degenerate equilibria,
%one may investigate the corresponding center (slow) manifold.
%We leave the issue of stability in future work. 


For the rest of the paper, we refer to the averaged data $\{(\mu_l, \bar{y}_l)\}_{l, u_l > 0}$ 
as the macroscopic data with respect to the sets $\{U_l\}$ \eqref{def:U-set}.
Also, we say a network is \emph{fully trained} if the parameter associated with it is a stationary point of the gradient flow dynamics \eqref{def:bias-gradflow}. 
An interesting feature of Lemma~\ref{lemma:critical} is that the equilibria depend only 
on averages of the training data defined in \eqref{cond:stationary}.
This means that if the training data were replaced by a smaller set which has the same average values defined in \eqref{cond:stationary}, then
the resulting equilibria are identical. 
This means that the network tends to fit an interpolant to this \emph{macroscopic} data
defined by \eqref{cond:stationary}.


Also, Lemma~\ref{lemma:critical} shows that 
%a fully trained network should interpolate 
%a set of macroscopic data
%and 
the partial sums of coefficients should be some quantities that are  determined by the training data. 
Moreover, Lemma~\ref{lemma:critical}  provides a training stopping criterion that can be used for determining the termination of gradient descent.



In Figure~\ref{fig:motivation-graph},
we provide an illustration of Lemma~\ref{lemma:critical}
using a simple task of fitting five training data $\{(\frac{k-3}{2},\frac{1-(-1)^k}{2})\}_{k=1}^5$
using a two-layer ReLU network of width $8$.
On the left, the fully trained network is plotted along with both the original training data ($\square$) and the macroscopic data ($\circ$).
As expected by Lemma~\ref{lemma:critical}, we see that 
the fully trained network interpolates the macroscopic data, which is identical to the original training data in this case.
On the middle, the trajectories of biases are plotted with respect to the number of epochs.
For reference, the original five training data points are also plotted as dashed-lines.
We first see that the two neurons located beyond $1$ are dead and remain unchanged.
We observe that all neurons saturate as the number of epochs increases, which indicates that the sets $\{U_l\}$ remain trapped in a given stage. 
On the right, the trajectories of coefficients are plotted.
We see that non of them vanishes. 
Since the sets $\{U_l\}$ remain unchanged and all the coefficients are not vanishing as the number of epochs increases, as expected by Theorem~\ref{thm:convergence}, 
we observe the convergence of both biases and coefficients. 
To this end, we see that the fully trained network for this simple task is represented by the sum of five macroscopic neurons: 
$f^{\text{NN}}(x) = 4\phi(x-0.5)- 4\phi(x)+4\phi(x+0.5)+c_2\phi(x+1) +c_1\phi(x-b_1)$,
%\begin{equation*}
%f^{\text{NN}}(x) = 4\phi(x-0.5)- 4\phi(x)+4\phi(x+0.5)+c_2\phi(x+1) +c_1\phi(x-b_1),
%\end{equation*}
where $c_2\phi(x+1)$ is represented by the sum of two neurons (green, yellow),
and $c_1\phi(x-b_1)$ corresponds to the neuron colored orange.
%,and $c_1+c_2 = -2$ (by Lemma~\ref{lemma:critical}).
\begin{figure}[htbp]
	\centerline{
		\includegraphics[width=4.3cm]{Figures/Ntr5_W8_Graph.pdf}
		\includegraphics[width=4.3cm]{Figures/Ntr5_W8_BiasRecords_data.pdf}
		\includegraphics[width=4.3cm]{Figures/Ntr5_W8_CoeffRecords.pdf}
	}
	\caption{Training results observed for fitting five training points
		with a two-layer ReLU network of width 8.
		The gradient decent is applied with a constant learning rate of $10^{-3}$.
		(Left) The final trained network.
		(Middle) The bias trajectories with respect to the number of epochs 
		along with the training input data (dashed lines).
		(Right) The coefficient trajectories with respect to the number of epochs.
	}
	\label{fig:motivation-graph}
\end{figure}



%Lemma~\ref{lemma:critical} gives 
%the necessary and sufficient conditions for
%a stationary point.
%%,
%however, it does not give qualitative descriptions of fully trained networks.
%With the aid of 

The following theorem shows that the fully trained networks
can be described in terms of multiple least squares regression lines.

\begin{theorem} \label{thm:LSQ-Stationary}
	Let $(\bm{b}^*, \bm{c}^*)$ be a stationary point of the gradient flow dynamics \eqref{def:bias-gradflow}.
	Without loss of generality, let ${b}^*_l \le {b}^*_{l+1}$ for all $l$.
	For each $l$ with $u_l \ne 0$, 
	let $\{(x_s^l, \hat{y}^l_s)\}_{s=1}^{u_l}$ be a set of modified training data 
	where $(x_s^l, y_s^l) \in U_l$ and
	\begin{align*}
	\hat{y}_s^l = y_s^l - \sum_{j=1}^{l-1} c_j^*\phi(x_s^l - b_j^*),\quad \forall s= 1,\cdots, u_l.
	\end{align*}
	Then, for each $l$ with $u_l \ge 2$, $\ell_{LSQ}(x) = c^*_l(x -b^*_l)$ is the least squares regression line
	obtained by the data set $\{(x_s^l, \hat{y}^l_s)\}_{s=1}^{u_l}$.
	And for each $l$ with $u_l = 1$, there exists $\alpha_l \in \mathbb{R}$ such that 
	$c^*_l=	\alpha_l + \frac{x_1^l\hat{y}^l_1}{1+(x_1^l)^2}$ and
	$b^*_lc^*_l = \alpha_l x^l_1 -\frac{\hat{y}^l_1}{1+(x_1^l)^2}$.
\end{theorem}
\begin{proof}
	The proof can be found in Appendix~\ref{app:thm:LSQ-Stationary}.
\end{proof}


%
%Analyzing  $\{U_l\}$ provides a way to characterize the set $\Omega$ of the stationary points of the gradient flow system \eqref{def:bias-gradflow}.
%Let $\textbf{k} = (k_1,\cdots,k_n)$ be a multi-index satisfying $0 \le k_l \le m$ and $\sum_{l=1}^n k_l = m$.
%We partition the set $\Omega$ of the stationary points by 
%\begin{equation*}
%	\Omega_{\textbf{k}} = \left\{(\bm{b},\bm{c}) \in \Omega |  \{U_l\}_{l=1}^n \text{ generated by } (\bm{b},\bm{c}) \text{ satisfy } u_l = k_l, \forall l \right\}.
%\end{equation*}
%It then readily follows from Theorem~\ref{thm:LSQ-Stationary} 
%that if $\textbf{k}$ satisfies $k_l \ge 2$ for all $l$,
%the set $\Omega_{\textbf{k}}$ contains at most one stationary point.




Theorem~\ref{thm:LSQ-Stationary} shows that 
a fully trained network consists of consecutive least squares regression lines, each of which is obtained by 
fitting the modified data from one of sets in $\{U_l\}$.
Also, the neurons whose corresponding $U_l$ is empty
connect least squares lines without incurring discontinuities. 


In conclusion, one may construct a fully trained neural network by gluing these least squares lines.
An explicit construction of such a network can be done by introducing extra neurons for
the purpose of gluing as described in Appendix~\ref{app:explicit-FTN}.
However, the construction may introduce seemingly artificial spikes. As a matter of fact, in Figure~\ref{fig:FullyTrained}, we illustrate the explicitly construction (Proposition~\ref{thm:fullyNN})
on the same learning task used in Figure~\ref{fig:motivation2}.
%, i.e., approximating $\sin(5\pi x)$ using 500 equidistant points.
The sets $\{U_l\}$ are obtained from the initial bias vector, which is randomly generated from the normal distribution $N(0,\sigma^2 I_n)$, where $\sigma = \sqrt{2}$ and $n=100$.
We clearly see that the resulting network contains many spikes and does not approximate the target function very well. 
However, we emphasize that it is a fully trained network 
and no further improvement would be obtained by continuing the gradient descent.

%any artificial gluing lines.
\begin{figure}[htbp]
	\centerline{
%		\includegraphics[width=6.5cm]{Figures/LSQ_sinPI_W10N500.pdf}
		\includegraphics[width=8cm]{Figures/LSQ_sin5PI_W100N500.pdf}
	}
	\caption{A fully trained ReLU network by Proposition~\ref{thm:fullyNN}
		for approximating  $\sin(5\pi x)$.
		The sets $\{U_l\}$ are generated by the bias vector from $N(0,\sigma^2 I_n)$,
		where $\sigma = \sqrt{2}$, $I_n$ is the identity matrix of size $n$, and $n= 100$.
		The biases are marked as crosses.
		The least squares lines and the gluing lines are shown as solid and dashed lines, respectively. 
		The target function is shown as dotted line. 
	}
	\label{fig:FullyTrained}
\end{figure}




%Conversely, given any partition of the interval containing all the training data points,
%one can directly construct a fully trained network without implementing gradient descent training.






%For reader's convenience, here we provide an algorithm that finds 
%a fully trained network constructed in the proof of Theorem~\ref{thm:fullyNN}.
%
%\begin{algorithm}
%	\caption{Active Neuron Training for univariate Shallow ReLU networks}
%	\label{alg:fullyNN}
%	\begin{algorithmic}[1]
%		\STATE{Input $\bm{b}^{(0)}, \bm{c}^{(0)}$, $k=0$, $M_0$, $M$=Maxepochs, Maxiter}
%		\WHILE{$k <$ Maxiter}
%		\STATE\label{line3}{Apply Gradient Descent starting at $(\bm{b}^{(k)},\bm{c}^{(k)})$ with $M_0$-epochs.}
%		\STATE{Output: $(\bm{b}_{M_0}^{(k)},\bm{c}_{M_0}^{(k)})$.}
%		\STATE{For each active neuron from $\bm{b}_{M_0}^{(k)}$,
%		perturbing only one 
%		find the best perturbation $\bar{\bm{b}}^{(k)}_{M_0}$.}
%		\STATE{Update $T := T \cup \{ \bigcup_{t\in\tau} t : \tau\in T_{C^\prime}{\setminus}
%			\mathcal{L}(T_{C^\prime})\}$}
%		\STATE{$k = k + 1$}
%		\ENDWHILE
%		\RETURN $(\bm{b}_*, \bm{c}_*)$
%	\end{algorithmic}
%\end{algorithm}







==> Submitted Version as of 07132020/introduction.tex <==
\section{Introduction} \label{sec:intro}
Neural networks are a key component in machine learning \cite{Lecun_Nature15_DeepLearning}.
The ability of neural networks to provide `best in class' approximation 
across a wide range of applications
has been the subject of intensive research \cite{Cybenko_MoC89, Barron_IEEE93, Mhaskar_Neurl96, Pinkus_Acta99, Yarotsky_NN17, Petersen_NN18}.
Nevertheless, the powerful expressivity of neural networks 
comes to naught if one is unable to effectively train (choose)
the parameters defining the network.
In general, neural networks are trained by gradient descent type optimization methods, or a stochastic variant thereof \cite{Ruder_16_GDoverview}.
The compositional structure of networks
combined with nonlinear activation functions
makes the associated optimization problem
non-convex.
Empirical evidence shows that,
despite the non-convex nature of the optimization problem,
such methods often manage to find a good enough solution
for the purposes of practical machine learning applications.
Nevertheless, the convergence of gradient descent methods
is often extremely slow and in many cases the error,
or loss, tends to remain at or above a level of 0.1-1\% relative error,
even when an extremely large number of steps are taken.
The fact that such methods have been
implemented extremely efficiently on state of the art computer hardware
helps ameliorate the problem to a large extent \cite{Abadi_16_TF,Paszke_19Pytorch}.
However, the fact remains that the training of neural networks 
using gradient descent, stochastic gradient descent, \texttt{Adam} \cite{kingma2014adam}, etc.
very probably accounts for more computer cycles than almost any other
application in scientific computing at the present time. 


Some investigations have been undertaken
to try to understand the behavior of gradient descent training of neural networks.
Several works \cite{allen2018convergence,du2018gradient-shallow,du2018gradient-DNN,oymak2019towards,zou2018stochastic,Jacot_18NTK} analyzed neural networks
in the so-called \emph{lazy} \cite{Chizat_19_LazyTrain}
(also known as, over-parameterized or kernel) regime,
where the number of network parameters is significantly larger than the number of training data, where it was shown that
gradient descent can train 
neural networks to interpolate all the training data (give a zero training loss).
However, as argued in  \cite{Chizat_19_LazyTrain, Lee_19_WideLinear}, lazy training is akin to simple linear regression type (kernel) learning, is inherently non-unique  and 
can lead to overfitting  \cite{Ghorbani_19_LimitationsLazy}.
In a similar vein \cite{Mei_PNAS18_MFland,Rotskoff_18_NNsInteracting,Sirignano_20_MFANNs} studied neural networks in the mean-field regime, where
the width of networks tends to infinity and, once again, it was shown that under certain conditions, a zero loss can be achieved.
While such limiting cases may be of interest in some machine learning applications, the adaptive regime \cite{Williams_NIPS19GDofShallow},
in which the amount of data exceeds the number of parameters in the model, is generally of more interest in practice. 



When neural networks belong to the adaptive regime,
we still lack a thorough understanding of gradient descent training of neural networks
and
%the loss surface is generally non-convex and 
%admits many local minima and/or flat regions. 
many questions remain elusive: Will the network converge to a `good' solution? 
Will convergence even occur at all \cite{Montavon_12_NNtricks}?
%there are many empirically observed training behaviors \cite{Maennel_18_GDquantizesReLU} including the plateau phenomenon \cite{Yoshida_NIPS19Data-Depend-PP}.
In practice, it is often observed 
that the loss function decreases rapidly at the beginning of training
but then, after a relatively small number of steps, significantly slows down.
The loss may even appear to stagnate over the period of a large number of epochs, only to then suddenly start to decrease
fast again for no apparent reason. 
This so-called \emph{plateau phenomenon} \cite{Fukumizu_00_Plateaus}
manifests itself in many learning tasks
and is seen even in quite simple applications.
For instance, suppose we wish to approximate $\sin(5\pi x)$ using a two-layer rectified linear unit (ReLU) network of width $100$ over $500$ equidistant training data points on $[-1,1]$.
For the training, we apply the gradient descent on the mean squared loss with a constant learning rate of $10^{-3}$.
% and set the maximum number of epochs to $10^{8}$.
In Figure~\ref{fig:motivation}, the loss versus the number of epochs is plotted during different training regimes.
%: Phase 1 is the period of upto $10^4$ epochs from the initialization, Phase 2 is the period of upto $3\times 10^7$ epochs from the end of Phase 1, and Phase 3 is the rest from the end of Phase 2. 
Figure~\ref{fig:moti:a} shows the behavior early in the training in which
the loss decreases quickly but then appears to saturate.
The unseasoned practitioner may even be tempted to terminate the training at this point believing convergence has been achieved.
However, if the gradient decent is continued, as shown in Figure~\ref{fig:moti:b}
the loss suddenly begins to decrease rapidly before again saturating at around $10^7$ epochs.
Continuing the gradient decent further as in Figure~\ref{fig:moti:c}, we observe a similar behavior repeated.
\begin{figure}[htbp]
	\centerline{
	\subfloat[ ]{\label{fig:moti:a}
	\includegraphics[height=3.3cm]{Figures/TEST04_W100N500Equi_GD1e8_Loss_scale1.pdf}
	}
	\subfloat[ ]{\label{fig:moti:b}
		\includegraphics[height=3.3cm]{Figures/TEST04_W100N500Equi_GD1e8_Loss_scale2.pdf}
	}	
	\subfloat[ ]{\label{fig:moti:c}
		\includegraphics[height=3.3cm]{Figures/TEST04_W100N500Equi_GD1e8_Loss_scale3.pdf}
	}
	}
	\caption{Training loss versus the number of epochs for approximating $\sin(5\pi x)$ with a two-layer ReLU network of width 100 using 
		500 equidistant training data on $[-1,1]$.
		Gradient decent (full-batch) is applied with a learning rate of $10^{-3}$.
	}
	\label{fig:motivation}
\end{figure}

This behavior has been observed by other researchers 
\cite{Saad_PhyRE95, Fukumizu_00_Plateaus} and termed ``plateau phenomenon" \cite{Park_NN00}.
Plateau phenomena not only make it difficult to decide at which stage one should terminate the gradient descent, but also means that convergence is very slow
with increasingly large numbers of seemingly unnecessary iterations 
spent in traversing a plateau only to enter a new regime in which the loss decreases rapidly.
Although \cite{Fukumizu_00_Plateaus,Cousseau_08_dynamics,Wei_08_dynamics,Guo_18_influence,Yoshida_NIPS19Data-Depend-PP}
provided some heuristic and empirical explanations on the cause of the plateau phenomenon,
a rigorous mathematical understanding is still lacking.



%{\bf Contribution.}
One of the aims of the present work is to identify and quantify the root causes of plateau phenomena. 
In order to isolate extraneous effects, we confine our attention to 
univariate two-layer ReLU networks
%,we confine our attention to this simple case 
where, as seen in the above example,
the phenomenon already exhibits itself.
We give a mathematical characterization of
the plateau phenomenon.
No assumptions are made on the number of neurons relative to the number of training data, and our results hold for both the lazy and adaptive regimes.
However, for the reasons mentioned before, 
we are mainly interested in the adaptive regime.


The main findings in the present work are summarized as follows:
\begin{itemize}
	\item 
	Plateaux correspond to periods during which
	\textit{activation patterns} remain constant (Theorem~\ref{thm:conti-loss-n}).
	The term activation pattern is defined below, but roughly speaking, refers to 
%	the relations between the network parameters (biases) and the training data points, that shows 
	the number of data points that activate a given neuron.
	\item We quantify the convergence of the gradient flow dynamics (Theorem~\ref{thm:convergence});
	give necessary and sufficient conditions for the stationary points (Lemma~\ref{lemma:critical}); and,
	relate fully trained networks to local least squares regression lines (Theorem~\ref{thm:LSQ-Stationary}) over subsets of the training data.
	\item
	Finally, based on these conclusions, 
	we propose a new iterative training method, Active Neuron Least Squares (ANLS), which is designed to avoid 
	the plateau phenomenon altogether (Section~\ref{sec:method}).
%	\item 
%	the fully trained networks interpolate a set of macroscopic data.
%	Here, a fully trained network refers to a network whose 
%	parameter is a stationary point of gradient flow dynamics.
\end{itemize}




The results of applying ANLS to the 
same learning task used in Figure~\ref{fig:motivation}
are shown in Figure~\ref{fig:motivation2}.
Figure~\ref{fig:moti2:a} shows 
the loss versus the number of iterations compared with gradient descent,
while Figure~\ref{fig:moti2:b} shows the fully trained neural networks.
\begin{figure}[htbp]
	\centerline{
		\subfloat[ ]{\label{fig:moti2:a}
			\includegraphics[width=6.3cm, height=4.5cm]{Figures/TEST04_W100N500Equi_Loss.pdf}
		}
		\subfloat[ ]{\label{fig:moti2:b}
			\includegraphics[width=6.3cm, height=4.5cm]{Figures/TEST04_W100N500Equi_Graph.pdf}
		}
	}
	\caption{Left: Training loss obtained by gradient descent (GD) and the proposed method (ANLS) versus the number of epochs on the same learning task used in Figure~\ref{fig:motivation}.
	Right: The fully trained neural networks by both GD and ANLS.
	}
	\label{fig:motivation2}
\end{figure}

While the ANLS method utilizes a least squares solution step to determine the linear parameters $\bm{c}$, this is not the reason that it avoids plateau phenomenon.
%, we mention some of related works on least squares based training of neural networks.
%The variable projection 
%\cite{Golub_Pereyra_73_NLSQ_vs, GolubLeVeque1979, Golub_Pereyra_03_Separable}, dated back to 1970s, is a method to solve separable nonlinear least square problems
%and it can be applied to train neural networks with the square loss \cite{Pereyra_06_VPonNN}.
% employed the variable projection method to train 
%two-layer neural networks with smooth activation functions.
Indeed, 
\cite{Cyr_19BoxInit} proposed a hybrid method that alternates between gradient descent and least squares, yet (as we will see) still exhibits plateau phenomena for essentially 
the same reasons as for pure gradient descent. 
%\cite{Fokina_19_Axons} proposed a greedy algorithm that generates adaptive neurons
%based on least squares. 
The key feature of ANLS that sets it aside from alternative approaches
is the \emph{explicit adjustment of the activation pattern at each step},
which is designed to enable a quick exit from a plateau region.
An algorithm based on complete orthogonal decomposition \cite{Golub_Book12_Matrix}
is presented which enables one to efficiently identify the optimal adjustment to the activation patterns.


The rest of this paper is organized as follows. 
After describing the model problem in section~\ref{sec:setup},
we present the gradient flow analysis in section~\ref{sec:GDflow}.
The proposed active neuron least squares is presented in section~\ref{sec:method}.
Numerical examples are provided in section~\ref{sec:example} to demonstrate 
our theoretical findings and illustrate the effectiveness of the proposed method.




%\noindent\fbox{%
%	\parbox{\textwidth}{%
%		YS: If needed, I will add more literature. But I found that most of them are not directly relevant to the current work.}%
%}
%%The two-layer ReLU network is relatively a well-studied model in deep learning literature. 
%{\bf Further related works on two-layer ReLU networks}
%\textcolor{red}{Remark: 
%	\cite{Williams_NIPS19GDofShallow} also analyzed the uni-variate two-layer ReLU networks in the lazy regime. 
%	However, I am not sure what is their main contribution. 
%	It seems to me that they aimed to investigate a bunch of things but ended up with having no affirmative results.
%	I think the work of \cite{Maennel_18_GDquantizesReLU} is the most relevant to our work if their proof is correct.
%	It seems to me that their analysis is not rigorously written and is hard to follow. I read this paper multiple times, but I think it contains many questionable statements and many jumps here and there in their proof.
%	However, their conclusion seems to be relevant to ours.}
%





==> Submitted Version as of 07132020/macroscopic.tex <==
\section{Training with Macroscopic Data}
Lemma~\ref{lemma:critical} shows that once the gradient flow dynamics reach at a stationary point, its corresponding network should interpolate a certain macroscopic data that consists of at most $n$ averaged points.
Motivated by this result, we propose a novel training scheme that not only accelerates the training but also reduce computational costs drastically.

\textcolor{red}{Thinking a way to extend this idea to a general deep ReLU network. I}

==> Submitted Version as of 07132020/method.tex <==
\section{Avoidance of Plateau Phenomenon} \label{sec:method}
Based on the insights learned in the previous section,
we propose a new training method that avoids the plateau phenomenon.
The main idea is to incorporate a mechanism whereby the training algorithm
can exit a plateau region within a single iteration. 
%if it appears that the plateau (or, equally well, activation pattern)
%may 
The proposed method is iterative and gradient-free. 
At each iteration, the method systematically generates a set of candidate parameters and selects the one with the smallest loss. 
%This is done by solving multiple least squares problems.

%The proposed method escapes the plateau region by systematically changing 
%the activation patterns at every iteration. 



\subsection{Rank-Deficient Least Squares Problem}
Firstly, suppose that a bias vector is given,
leaving one with the task of minimizing the loss \eqref{def:Loss}
with respect to $\bm{c}$.
The corresponding coefficients are obtained by solving the least squares problem
\begin{equation*} 
	\min_{\bm{c}} \|\bm{A} \bm{c} - \bm{y}\|^2, \qquad [\bm{A}]_{ij} = \phi(x_i - b_j), \qquad \bm{y} = \begin{bmatrix}
	y_1 \\ \vdots \\ y_m
	\end{bmatrix}.
\end{equation*}
We are primarily interested in the adaptive region in which the amount of data exceeds the number of neurons. 
%Thus, the system matrix $\bm{A}$ is over-determined. 
Furthermore, owing to the ReLU activation function $\phi$, the matrix $\bm{A}$ is often rank deficient. We are therefore faced with 
a rank deficient least squares problem which has infinitely many solutions.
We regularize by seeking the minimum norm solution:
\begin{equation} \label{def:LSQ}
	\bm{c}_{\text{LSQ}} \impliedby \min_{\bm{c} \in \mathcal{S}} \|\bm{c}\|, \qquad
	\mathcal{S} = \left\{\bm{c} \in \mathbb{R}^n : \|\bm{A}\bm{c} - \bm{y}\| = \min_{\tilde{\bm{c}}} \|\bm{A}\tilde{\bm{c}} - \bm{y}\|  \right\}.
\end{equation}
The solution to the problem is given by $\bm{c}_{\text{LSQ}} = \bm{A}^{\dagger}\bm{y}$, where $\bm{A}^{\dagger}$ is the Moore–Penrose inverse of $\bm{A}$.


If the solution satisfies the linear system exactly, 
a zero training loss is obtained and 
the resulting parameter $(\bm{b},\bm{c}_{\text{LSQ}})$ produces a fully trained network.

%\textit{Remark:} If the number of neurons is greater than or equals to the number of training data,
%one can explicitly construct a piece-wise linear interpolation,
%which leads a zero training loss.
%No training is needed in this case.
%Hence, we are mainly interested in the adaptive regime.
 
\subsection{Generating candidate pairs} \label{subsec:generating}
As shown in Theorem~\ref{thm:conti-loss-n}, each plateau 
corresponds to a period during which the activation patterns do not change.
As demonstrated in Figure~\ref{fig:motivation}, 
the main cause of the slow down of gradient descent training
is the time spent in traversing a plateau before entering a new one. 
In order to quickly exit such a plateau, 
the activation patterns \eqref{def:U-set} have to change.
%To this end, given a bias vector $\bm{b}$, 
%However, since there are infinitely many such biases, there is no trivial way of doing so. 
To this end, given a bias vector $\bm{b}$,
we seek for a candidate bias, which produces different activation patterns. 
We make the following rules to generate candidate bias vectors.



Let $\bm{b} = [b_1,\cdots, b_n]^T$ be a given bias vector such that  $b_1 < \cdots < b_n$.
We say  $\bm{b}'=[b_1',\cdots,b_n']^T$ is a candidate bias vector with respect to $\bm{b}$ if the following rules are satisfied:
\begin{enumerate}
	\item  $b_j' = b_j$ for all $j$ but one. That is, we only change one neuron at a time. 
	\item 
	$b_1' < \cdots < b_n'$.
	That is, we do not move a neuron in a way that the bias ordering is violated. 
	\item 
	Let $\{U_l\}$ and $\{U_l'\}$ be the sets defined in \eqref{def:U-set} by $\bm{b}$ and $\bm{b}'$, respectively. 
	If the $k$-th neuron has changed, i.e., $b_k \ne b_k'$, 
	we have $|U_k| = |U_k'|  \pm 1$.
	\item If $U_l = \emptyset$ for all $l \ge k$, 
	then $b_l' = b_l$ for all $l \ge k$. That is,
	we do not move dead neurons.
	\item 
	If $U_l = \emptyset$ for all $l > k$ and $U_k \ne \emptyset$,
	then $U_k' \ne \emptyset$. 
	That is, we do not move a neuron in a way that the neuron is dead.
	\item 
	Suppose $b_k' \ne b_k$. Then, 
	$b_k'$ is one of three points:
	(i) the middle point of two data points,
	(ii) the middle point of a data point and $b_k$,
	or (iii) the smallest data point minus a fixed small number, say, $10^{-8}$.
\end{enumerate}
For each candidate bias vector, one can solve 
the least squares problem \eqref{def:LSQ} to find its corresponding optimal coefficient vector.
This generates a single candidate pair. 
%We then choose the best pair, denoted by $\bm{\theta}_{BC}$,  that results in the smallest loss value.
%If the loss by the best candidate pair is greater than 
%the loss by the current pair, 
%we return the current pair and terminate the process.

We illustrate the generation of candidate bias vectors in Figure~\ref{fig:candidate-ex}
where there are 5 neurons and 10 data points.
It can be seen that there are two locations that the first neuron (far left) could be located
and each location generates a candidate bias vector, while fixing all the other neurons.
Since $U_2$ is empty, there is only one location that the second neuron could be located. 
Similarly, the third- and the fourth neurons generate one and two candidate vectors, respectively.    
Finally, since $U_5$ contains only one training data point, 
if the fifth neuron were located beyond the point in $U_5$,
it will not be activated by all the points and become dead. 
Thus, the fifth neuron can generate only one candidate vector by moving itself to the left.
By counting all the cases, we see that there are total of 7 candidate bias vectors generated by our rules.
\begin{figure}[htbp]
	\centerline{
		\includegraphics[width=13cm]{Figures/Candidate.png}
	}
	\caption{Illustration of generating candidate biases by our rules for $n=5$.
		The red dots ($\textcolor{red}{\bullet}$) show the current positions of the biases $\{b_j\}$.
		The blue dots ($\textcolor{blue}{\bullet}$) show the feasible positions of the biases.
		The cross marks ($\textcolor[rgb]{0.4392, 0.1882, 0.6275}{\text{\ding{54}}}$) show the positions of the training points $\{x_k\}_{k=1}^{m}$ for $m=10$.
	}
	\label{fig:candidate-ex}
\end{figure}

\subsection{Active Neuron Least Squares} \label{subsec:ANLS}
Given $\bm{b}^{(k)}$, 
by solving the least squares problem \eqref{def:LSQ},
its corresponding optimal coefficient vector $\bm{c}_{\text{LSQ}}^{(k)}$ is obtained.
Let 
$\bm{\theta}^{(k)}_{\text{LSQ}} = (\bm{b}^{(k)}, \bm{c}_{\text{LSQ}}^{(k)})$. 
Let $\bm{b}^{(0)}$ be an initialization of the bias vector.
Starting at $k = 0$, the following steps are repeatedly conducted until converge:
\begin{itemize}
	\item Step 1: 
	By following the rules described in section~\ref{subsec:generating}, generate all the possible candidate pairs with respect to  $\bm{b}^{(k)}$.
	Find the best candidate pair $\bm{\theta}^{(k)}_{\text{BC}} = (\bm{b}_{\text{BC}}^{(k)}, \bm{c}_{\text{BC}}^{(k)})$ that results in the smallest loss.
	\item Step 2: 
	If $\mathcal{L}(\bm{\theta}^{(k)}_{\text{LSQ}}) \le \mathcal{L}(\bm{\theta}^{(k)}_{\text{BC}})$,
	terminate the process and return $\bm{\theta}^{(k)}_{\text{LSQ}}$.
	Else, set $\bm{b}^{(k+1)}:= \bm{b}_{\text{BC}}^{(k)}$
	and back to Step 1 with $k \to k+1$.
\end{itemize}


We call the proposed method as the \emph{active neuron least squares} (ANLS). 
By the construction of the method, the convergence of the loss by ANLS readily follows.
\begin{proposition} \label{prop:ANLSQ-convg}
	Let $\{\bm{\theta}^{(k)}_{\text{LSQ}} \}_{k\ge 1}$ be a sequence of parameters
	generated by the active neuron least squares.
	Then, 
	$
	\lim_{k \to \infty} \mathcal{L}(\bm{\theta}_{\text{LSQ}}^{(k)}) = L^*
	$
	for some $L^* \ge 0$.
%	Furthermore, there exists a convergent subsequence $\{\bm{\theta}^{(k_l)} \}_{l\ge 1}$.
\end{proposition}
\begin{proof}
	Suppose for all $k$, $\mathcal{L}(\bm{\theta}^{(k)}_{\text{BC}}) < \mathcal{L}(\bm{\theta}^{(k)}_{\text{LSQ}})$.
	Unless, the proof is done. 
	Since $\{\mathcal{L}(\bm{\theta}_{\text{LSQ}}^{(k)})\}_{k \ge 0}$ is a monotone decreasing sequence that is bounded below, 
	we have the convergence of the loss.
%	: There exists $L^*$ such that 
%	\begin{align*}
%		\lim_{k \to \infty} \mathcal{L}(\bm{\theta}^{(k)}) = L^*, \qquad 0 \le L^* <  \mathcal{L}(\bm{\theta}^{(0)}).
%	\end{align*}
%	Let $A^k_{\text{BC}}$ and $A^k_{\text{LSQ}}$
%	be the system matrices generated by $\bm{\theta}^{(k)}_{BC}$ and $\bm{\theta}^{(k)}_{LSQ}$,
%	respectively.
%	Then,
%	$\mathcal{L}(\bm{\theta}^{(k)}_{\text{BC}}) < \mathcal{L}(\bm{\theta}^{(k)}_{LSQ})$
%	is equivalent to
%	$$
%	\|\bm{y} - \Pi_{A^k_{\text{BC}}}\bm{y}\| < \|\bm{y} - \Pi_{A^k_{\text{LSQ}}}\bm{y}\|.
%	$$
%	Note that $A^k_{\text{BC}}$ and $A^k_{\text{LSQ}}$ share
%	all the columns but one, say $l$-th column.
%	For a matrix $V$, let ${}_{l}\check{V}$ be a submatrix of $V$ obtained by deleting the $l$-th column.
%	Thus, 
%	the $l$-th column of $A^k_{\text{BC}}$
%	cannot be in the column space of ${}_{l}\check{A}^k_{\text{LSQ}}$.
%	
%	By the construction, the bias vector is bounded both above and below.
%	Also, since \textcolor{red}{the coefficient vector is the minimum norm solution to 
%	the least squares problem \eqref{def:LSQ}, it is also uniformly bounded. }
%	Therefore, there exists a convergent subsequence $\{\bm{\theta}^{(k_l)} \}_{l\ge 1}$.
%	\begin{align*}
%		\lim_{l \to \infty} \bm{b}^{(k_l)} = \bm{b}^*
%%		\implies
%%		\lim_{l \to \infty} \bm{c}_{\text{LSQ}}^{(k_l)} = \bm{c}_{\text{LSQ}}^*,
%	\end{align*}
%	where the implication holds because the coefficient vector is determined by solving the least squares problem (least-norm) by fixing the bias
%	and the least squares solution is continuous with respect to the system matrix.
\end{proof}


\subsection{Efficient Implementation}
The step 1 of ANLS requires one to solve multiple least squares problems to determine the best pair. 
This could be computationally expensive, especially when the number of data is large. 
We thus present an efficient implementation of Step 1 via complete orthogonal decomposition (COD) \cite{Golub_Book12_Matrix}.

For a matrix $\bm{A}$, let us denote the $i$-th row and the $j$-th column of $\bm{A}$
by $\bm{A}_{i,:}$ and $\bm{A}_{:,j}$, respectively.
\begin{theorem} \label{thm:LSQ}
	Let $\bm{A}$ be a matrix of size $m\times n$ with  $m \ge n$.
	Let us consider a COD of $\bm{A}$:
	\begin{align*}
		\bm{Q}^T\bm{AZ} = \hat{\bm{T}}, \quad
		\text{where} \quad 
		\hat{\bm{T}} = \begin{bmatrix}
		\bm{T} & \bm{0} \\ \bm{0} & \bm{0}
		\end{bmatrix},
		\quad r = \text{rank}(\bm{A}), 
		\quad
		\bm{Z} = \begin{bmatrix}
		\hat{\bm{Z}}, & \tilde{\bm{Z}}
		\end{bmatrix}
	\end{align*}
	$\bm{Q}\in \mathbb{R}^{m\times m}$ and $\bm{Z}\in\mathbb{R}^{n\times n}$
	are orthogonal matrices,
	$\bm{T} \in \mathbb{R}^{r\times r}$ is a triangular matrix,
	and $\hat{\bm{Z}} \in \mathbb{R}^{n\times r}$.
	Let $\bm{V}_l$ be a matrix of size $m\times n$ 
	whose entries are all zeros except for the $l$-th column.
	Let $\bm{v}_l$ be the $l$-th column of $\bm{V}_l$.
	Let 
	\begin{align*}
	\bm{Q}^T\bm{v}_l &= \begin{bmatrix}
	\bm{q}_l^{(1)} \\  \bm{q}_l^{(2)}
	\end{bmatrix}, 
	\quad
	\bm{Q}^T\bm{y} = 
	\begin{bmatrix}
	\bm{p}^{(1)} \\ \bm{p}^{(2)} 
	\end{bmatrix},
	\qquad 
	\bm{q}_l^{(1)}, \bm{p}^{(1)} \in \mathbb{R}^{r},
	\end{align*}
	and $\tilde{\bm{A}} = \bm{A} + \bm{V}_l$.
	Then, the solution to the least squares problem \eqref{def:LSQ} for $(\tilde{\bm{A}}, \bm{y})$ is given by 
	$
		\tilde{\bm{c}}_{\text{LSQ}} = \bm{Z}\begin{bmatrix}
		\bm{x}_l^{(1)} \\ \bm{x}_l^{(2)}
		\end{bmatrix}
	$,
	and its corresponding loss is
	\begin{align*}
	\|\tilde{\bm{A}}\tilde{\bm{c}}_{\text{LSQ}} - \bm{y}\|^2 =
	\begin{cases}
	\|\bm{p}^{(2)}\|^2 - \|\bm{q}_l^{(2)}\|^2(d_l^*)^2, &\text{if } \|\tilde{\bm{Z}}_{l,:}\| > 0 \\
	\|\bm{p}^{(2)}\|^2  + \|\bm{p}^{(1)}\|^2  - \bm{s}_l^T\bm{x}_l^{(1)},  &\text{if } \|\tilde{\bm{Z}}_{l,:}\| = 0
	\end{cases},
	\end{align*}
	where $d^*_l = \begin{cases}
	\frac{\langle \bm{p}^{(2)}, \bm{q}_l^{(2)}\rangle }{\|\bm{q}_l^{(2)}\|^2}, &\text{if } \|\bm{q}_l^{(2)}\| > 0 \\
	\hat{\bm{Z}}_{l,:}\bm{x}_l^{(1)} &\text{if } \|\bm{q}_l^{(2)}\| = 0
	\end{cases}$, 
	$\bm{x}_l^{(1)} = 
	\begin{cases}
	\bm{T}^{-1}(\bm{p}^{(1)} - d_l^*\bm{q}_l^{(1)}), & \text{if } \|\tilde{\bm{Z}}_{l,:}\| > 0 \\
	\bm{M}_l^{\dagger}\bm{s}_l, & \text{if } \|\tilde{\bm{Z}}_{l,:}\| = 0
	\end{cases}$,
	\begin{align*}
%	\bm{x}_l^{(1)} &= 
%	\begin{cases}
%	\bm{T}^{-1}(\bm{p}^{(1)} - d_l^*\bm{q}_l^{(1)}), & \text{if } \|\tilde{\bm{Z}}_{l,:}\| > 0 \\
%	\bm{M}_l^{\dagger}\bm{s}_l, & \text{if } \|\tilde{\bm{Z}}_{l,:}\| = 0
%	\end{cases}, 
%	\\
	\bm{x}_l^{(2)} &= 
	\begin{cases}
	\frac{d_l^* - \hat{\bm{Z}}_{l,:}\bm{x}_l^{(1)}}{\|\tilde{\bm{Z}}_{l,:}\|^2}(\tilde{\bm{Z}}_{l,:})^T,& \text{if } \|\tilde{\bm{Z}}_{l,:}\| > 0 \\
	\bm{0}, & \text{if } \|\tilde{\bm{Z}}_{l,:}\| = 0
	\end{cases}, 
%	\\
%	d^*_l &= \begin{cases}
%	\frac{\langle \bm{p}^{(2)}, \bm{q}_l^{(2)}\rangle }{\|\bm{q}_l^{(2)}\|^2}, &\text{if } \|\bm{q}_l^{(2)}\| > 0 \\
%	\hat{\bm{Z}}_{l,:}\bm{x}_l^{(1)} &\text{if } \|\bm{q}_l^{(2)}\| = 0
%	\end{cases}, 
	\end{align*}
	$\tilde{\bm{T}}_l = \bm{T} + \bm{q}_l^{(1)}\hat{\bm{Z}}_{l,:}$,
	$\bm{M}_l = \tilde{\bm{T}}_l^T\tilde{\bm{T}}_l + \|\bm{q}_l^{(2)}\|^2\hat{\bm{Z}}_{l,:}^T\hat{\bm{Z}}_{l,:}$, 
	and 
	$\bm{s}_l = \bm{T}^T \bm{p}^{(1)} + (\bm{y}^T\bm{v}_l)\hat{\bm{Z}}_{l,:}^T$.
\end{theorem}
\begin{proof}
	The proof can be found in Appendix~\ref{app:thm:LSQ}.
\end{proof}

\textit{Remark 1:} 
Let $\bm{b}'$ be a candidate bias vector with respect to $\bm{b}^{(k)}$, which only differs by the $l$-th entry.
By applying Theorem~\ref{thm:LSQ} with $[\bm{v}_l]_j = \phi(x_j - b'_l) - \phi(x_j - b_l^{(k)})$,
one can obtain the candidate pair and its corresponding loss.

\textit{Remark 2:} 
Since $\|\bm{y}\|^2 = \|\bm{p}^{(1)}\|^2 + \|\bm{p}^{(1)}\|^2$
and $\|\bm{v}_l\|^2 = \|\bm{q}_l^{(1)}\|^2 + \|\bm{q}_l^{(2)}\|^2$,
the first $r$ columns of $\bm{Q}$ in Theorem~\ref{thm:LSQ} is necessary
for the method.


\textit{Remark 3:} 
In the case where $\|\tilde{\bm{Z}}_{l,:}\| = 0$, 
the method still requires to solve a $r\times r$ linear system of equations.
However, this is a much smaller problem compared to the original least squares \eqref{def:LSQ}.

%\textit{Remark 4:} Theorem~\ref{thm:LSQ} can be used in more general cases

%\textit{Remark 4:} 
%The complexity of each iteration of the ANLS can be computed as follows.
%At each iteration, one needs to find a COD of a $m \times n$ matrix.
%We follows the two-step procedure \cite{Golub_Book12_Matrix}: (i) the QR-decomposition with column pivoting 
%and the QR-decomposition on a $n \times r$ matrix.
%Since the QR with column pivoting requires $4mnr - 2r^2(m+n) + 4r^3/3$ flops
%and the QR factorization requires $2nr^2 - 2r^3/3$,
%also, computing $Q$ requires
%Thus, a COD requires 
%\begin{align*}
%&(4mnr - 2(m+r)n^2 + 4n^3/3) + (4mnr - 2r^2(m+n) + 4r^3/3) \\
%&= 8mnr -2(mn^2+rn^2+mr^2+nr^2) + 4(n^3+r^3)/3 \\
%&(4nr^2 - 2r^2(n+r) + 4r^3/3) + (2nr^2 - 2r^3/3) \\
%&= 6nr^2 - 2(n+r)r^2 + 2r^3/3
%\end{align*}
%The total complexity is 
%\begin{align*}
% 4(n^3/3 + mnr) - 2nr(n-r) -2m(n-r)^2 + \text{num of perturbation of second kinds}\mathcal{O}(r^3) 
%\end{align*}

%We remark that the work of \cite{Cyr_19BoxInit} proposed a training method that utilizes the least squares problem for the coefficient vector. 
%However, the ANGD is a different approach in the following sense:
%Firstly, solving the linear system \eqref{cond:stationary} is not the same as
%solving the least squares problem that is obtained from minimizing the square loss function
%assuming the bias vector is fixed. 
%Secondly, Step 3 of the ANGD directly searches the best bias configuration 
%by perturbing one active neuron at a time. 
%This is motivated by Theorem~\ref{thm:conti-loss-n}.

%To demonstrate the performance of the method,
%let us consider the following learning task.
%\begin{figure}[htbp]
%	\centerline{
%		\includegraphics[width=6.3cm]{Figures/SEED1234_W8_Ntr5Intro_GD_lr1e-3_AN_numGD1_Loss.pdf}
%		\includegraphics[width=6.3cm]{Figures/SEED1234_W8_Ntr5Intro_GD_lr1e-3_AN_numGD1_Graph.pdf}
%	}
%	\caption{Training result observed for fitting five training points
%		with a shallow ReLU network of width 8.
%		For AN, we set $M_k = 1$ for all $k$.
%		The standard gradient decent method is applied with a constant learning rate of $10^{-3}$.
%		(Left) The training loss with respect to the number of gradient descent epochs.
%		(Right) The graphs of fully trained networks.
%	}
%	\label{fig:motivation-AN}
%\end{figure}
%
%
%
%The case where the number of training data is larger than the number of neurons.
%\begin{figure}[htbp]
%	\centerline{
%		\includegraphics[width=4.3cm]{Figures/SEED1234_W8_Ntr500Equi_AN_numGD10_init100_Graph.pdf}
%		\includegraphics[width=4.3cm]{Figures/SEED1234_W8_Ntr500Equi_GD_lr1e-3_AN_numGD10_init100_Loss.pdf}
%		\includegraphics[width=4.3cm]{Figures/SEED1234_W8_Ntr500Equi_GD_lr1e-3_Graph.pdf}
%	}
%	\caption{Training result observed for fitting five training points
%		with a shallow ReLU network of width 8.
%		The training data points are 500-equidistant points in $[-1,1]$.
%		For AN, we set $K=10$ and $M_k = 100$ for all $k$ but $M_K = 10^{6} - \sum_{k=0}^{K-1} M_k$.
%		The standard gradient decent method is applied with a constant learning rate of $10^{-3}$.
%		The graphs of fully trained networks by AN (left) and GD (right).
%		(Middle) The training loss with respect to the number of gradient descent epochs.
%	}
%	\label{fig:AN-W8N500}
%\end{figure}
%
%
%
%
%\begin{figure}[htbp]
%	\centerline{
%		\includegraphics[width=4.3cm]{Figures/SEED1234_W10_Ntr30Unif_AN_numGD10_init100_Graph.pdf}
%		\includegraphics[width=4.3cm]{Figures/SEED1234_W10_Ntr30Unif_GD_lr1e-3_AN_numGD10_init100_Loss.pdf}
%		\includegraphics[width=4.3cm]{Figures/SEED1234_W10_Ntr30Unif_GD_lr1e-3_Graph.pdf}
%	}
%	\caption{Training result observed for fitting five training points
%		with a shallow ReLU network of width 8.
%		The training data points are 30 uniform random points from $[-1,1]$.
%		For AN, we set $K=10$ and $M_k = 100$ for all $k$ but $M_K = 10^{6} - \sum_{k=0}^{K-1} M_k$.
%		The standard gradient decent method is applied with a constant learning rate of $10^{-3}$.
%		The graphs of fully trained networks by AN (left) and GD (right).
%		(Middle) The training loss with respect to the number of gradient descent epochs.
%	}
%	\label{fig:AN-W10N30}
%\end{figure}




%\begin{lemma} \label{lem:line-multiNeurons}
%	For $z, a, d \in \mathbb{R}$ and $a \ne 0$, let
%	\begin{equation*}
%	f_z(x) = (ax + d)\cdot \mathbb{I}_{x \ge z}(x).
%	\end{equation*}	
%	For any $\epsilon > 0$ and a positive integer $M$ greater than 1,
%	let $\{b_j\}_{j=1}^M$ be a partition of the interval $[z-\epsilon,z]$
%	with $b_1 = z-\epsilon$ and $b_M = z$.	
%	Then, $\forall x \in (-\infty,z-\epsilon]\cup [z,\infty)$,
%	\begin{equation}
%	f_z(x) = \sum_{j=1}^M c_j\phi(x - b_j),
%	\end{equation}
%	where
%	\begin{equation*}
%	\bm{c} = \begin{bmatrix}
%	c_1 \\
%	\vdots \\
%	c_M
%	\end{bmatrix}
%	= \frac{1}{M}\left[a\bm{1} +
%	\frac{a\mu_b + d}{\sigma_b^2}(\mu_b\bm{1} - \bm{b})\right], \qquad
%	\bm{1} = 
%	\begin{bmatrix}
%	1 \\ \vdots \\ 1
%	\end{bmatrix}, 
%	\quad
%	\bm{b} = \begin{bmatrix}
%	b_1 \\ \vdots \\ b_M
%	\end{bmatrix},
%	\end{equation*}
%	and $\mu_b$ and $\sigma_b^2$ are the mean and variance of $\bm{b}$.
%\end{lemma}
%\begin{proof}
%	For $\epsilon > 0$, if $0 \le z + \frac{d}{a} < \epsilon$,
%	the proof is completed.
%	To be filled.
%\end{proof}
%
%
%\textcolor{red}{need to be written more precisely.}
%First, note that for any bias vector $\bm{b}$,
%it follows from Lemma~\ref{lem:line-multiNeurons} that 
%one can construct a neural network that tries its best
%to be a fully-trained one. ($NN^*$)
%
%
%
%For an initial bias vector $\bm{b}^{(0)}$ and a set of training data,
%we identify the set of active neurons and construct a partition of the training points with respect to $\bm{b}^{(0)}$.
%There are at most two ways an active neuron can move; left and right.
%If an active neuron is moved either way, we construct a $NN^*$
%and compute two values.



==> Submitted Version as of 07132020/setup.tex <==
\section{Model Problem} \label{sec:setup}
Let us consider a univariate two-layer ReLU network
\begin{equation*}
f(x;\bm{\theta}) = \sum_{j=1}^n c_j\phi(w_jx-b_j), \qquad \bm{\theta} =  \{(b_j, c_j, w_j)\}_{j=1}^n,
\end{equation*}
where $\phi(x) = \max\{x,0\}$ is the rectified linear unit (ReLU) activation function.
%We denote the set of the input training data as $\mathcal{T}_m = \{x_i\}_{i=1}^m$.
%Since we consider the univariate model, let $x_1 < x_2 < \cdots < x_m$.
%For a finite set $A$, its cardinality is denoted by $|A|$.
Given a set of training data $\{(x_i,y_i)\}_{i=1}^m$, where $x_1 < x_2 < \cdots < x_m$,
we seek parameters $\bm{\theta}$ that minimize the loss function $\mathcal{L}$ defined by
\begin{equation} \label{def:Loss}
\mathcal{L}(\bm{\theta}) = \frac{1}{2}\sum_{i=1}^m (f(x_i;\bm{\theta})-y_i)^2,
\end{equation}
which measures the $\ell_2$ norm of the discrepancy between the output data and the prediction.
We shall see that many of the phenomena we wish to study
already manifest themselves in the special case where $w_j = 1$.
As a matter of fact, fixing $w_j=1$ does not change the expressivity of the neural networks, as shown by the following result:
\begin{proposition} \label{prop:w=1}
	Let $\Omega$ be a bounded interval and
	\begin{equation*}
	\begin{split}
	\mathcal{N} = \text{span}\{\phi(wx+b) | w, b \in \mathbb{R}, x \in \Omega \}, \qquad
	\mathcal{N}_{+} = \text{span}\{\phi(x+b) | b \in \mathbb{R}, x \in \Omega \}.
	\end{split}
	\end{equation*} 
	Then, $\mathcal{N} = \mathcal{N}_{+}$.
\end{proposition}
\begin{proof}
	Without loss of generality, let $\Omega=[0,1]$.
	Note that $\phi(wx+b) = \phi(b)$ if $w=0$
	and $\phi(wx+b) = |w|\phi(\text{sign}(w)(x+b/|w|))$ if $|w| \ne 0$.
	
	If $w=0$ and $b > 0$, observe that $\phi(b) = b = \phi(x + b) - \phi(x)$ for $x \in \Omega$.
	
	If $|w|\ne 0$, it suffices to show that any $\phi(-x+b)$ can be 
	expressed as a function in $\mathcal{N}_{+}$ on $\Omega$.
	Observing that 
	\begin{equation*} 
	\phi(-x+b) = \begin{cases}
	0, & \forall x \in \Omega, \text{if } b \le 0, \\
	\phi(x-b)-2\phi(x) + \phi(x+b), & \forall x \in \Omega, \text{if } b > 0
	\end{cases}
	\end{equation*}
	completes the proof.
\end{proof}

In view of Proposition~\ref{prop:w=1}, we may fix $w_j = 1$ for all $j$,
and consider networks of the form
\begin{equation} \label{def:NN}
f(x;\bm{b},\bm{c}) =\sum_{j=1}^n c_j\phi(x-b_j), \quad \text{where} \quad 
\bm{b} = \begin{bmatrix}
b_1 \\ \vdots \\ b_n
\end{bmatrix}, \quad
\bm{c} = \begin{bmatrix}
c_1 \\ \vdots \\ c_n 
\end{bmatrix}.
\end{equation}
The task of training the network is equivalent to selecting the positions of the nodes $\{b_j\}$ 
and the weights $\{c_j\}$
in a piecewise linear approximation \cite{He_etal_19ReLUFEM}. 
If the positions $\{b_j\}$ of the knots are specified, then the coefficients $\{c_j\}$ minimizing the loss can be obtained by solving a linear system of equations.
Here, however, we are also interested in determining the optimal knot placement which results in a highly non-linear minimisation problem for which we employ gradient descent to seek a minimum over both $\{b_j\}$ and $\{c_j\}$.

The network parameter $\bm{\theta} = \{(b_j,c_j)\}_{j=1}^n$ can be viewed as a vector in $\mathbb{R}^{2n}$.
% by concatenating two vectors $\bm{b}$ and $\bm{c}$.
%By treating $\bm{\theta}$ as a vector of length $2n$, 
Gradient descent proceeds iteratively starting with an initialization of the parameters $\bm{\theta}^{(0)}=\{(b_j^{(0)}, c_j^{(0)})\}_{j=1}^n$, and the $k$-th iteration updates the parameters according to the rule
$$
\bm{\theta}^{(k)} = \bm{\theta}^{(k-1)} - \eta_k \nabla_{\bm{\theta}} \mathcal{L}(\bm{\theta}^{(k-1)}), 
$$
where $\eta_k > 0$ is the learning rate at the $k$-th iteration
and $\nabla_{\bm{\theta}}$ denotes the gradient with respect to the free parameters $\bm{\theta}$.
In general, the learning rate should be chosen sufficiently small in order for the scheme to converge to a minimum.
In the limit $\eta_k \to 0$, we arrive at a continuous counterpart of the gradient descent scheme, in which the discrete iterates $\{\bm{\theta}^{(k)}\}$ are replaced by a function $\{\bm{\theta}(t), t \ge 0\}$
satisfying an initial value problem generated by the following system of first order autonomous ordinary differential equations (ODEs),
\begin{equation} \label{def:grad-flow}
\dot{\bm{\theta}}(t) = -\nabla_{\bm{\theta}} \mathcal{L}(\bm{\theta}(t)), \qquad 
\bm{\theta}(0) = \bm{\theta}^{(0)}.
\end{equation}
By the same token, the associated loss $\mathcal{L}(\bm{\theta}(t))$
may be regarded as a function of $t$ which, with a slight abuse of notation,
we shall henceforth denote as $\mathcal{L}(t)$.
Likewise, we shall speak of $t$ as a `time' although, strictly speaking, $t$ simply parameterizes the state of the system as the gradient descent updates proceed.

==> Submitted Version as of 07132020/shared.tex <==
% SIAM Shared Information Template
% This is information that is shared between the main document and any
% supplement. If no supplement is required, then this information can
% be included directly in the main document.


% Packages and macros go here
\usepackage{lipsum}
\usepackage{amsfonts}
\usepackage{amssymb}
\usepackage{graphicx}
\usepackage{epstopdf}
\usepackage{algorithmic}
\usepackage{enumerate}
\usepackage{verbatim,amscd}
\usepackage{latexsym, bm, float, color}
\usepackage{mathtools}
\usepackage{pifont}
\usepackage{subfig}

\ifpdf
  \DeclareGraphicsExtensions{.eps,.pdf,.png,.jpg}
\else
  \DeclareGraphicsExtensions{.eps}
\fi

% Add a serial/Oxford comma by default.
\newcommand{\creflastconjunction}{, and~}

% Used for creating new theorem and remark environments
\newsiamremark{remark}{Remark}
\newsiamremark{hypothesis}{Hypothesis}
\crefname{hypothesis}{Hypothesis}{Hypotheses}
\newsiamthm{claim}{Claim}



% Sets running headers as well as PDF title and authors
\headers{Plateau Phenomenon}{M. Ainsworth and Y. Shin}

% Title. If the supplement option is on, then "Supplementary Material"
% is automatically inserted before the title.
\title{Plateau Phenomenon in Gradient Descent Training of ReLU networks: Explanation, Quantification and Avoidance\thanks{Submitted to the editors 2020/07/14.
\funding{This work was funded by the PhILMS grant DE-SC0019453}}}

% Authors: full names plus addresses.
\author{Mark Ainsworth\thanks{Division of Applied Mathematics, Brown University, Providence, RI 02912
  (\email{mark\_ainsworth@brown.edu}, \email{yeonjong\_shin@brown.edu}).}
\and Yeonjong Shin\footnotemark[2]}


\usepackage{amsopn}
\DeclareMathOperator{\diag}{diag}


%%% Local Variables: 
%%% mode:latex
%%% TeX-master: "ex_article"
%%% End: 


==> macroscopic.tex <==
\section{Training with Macroscopic Data}
Lemma~\ref{lemma:critical} shows that once the gradient flow dynamics reach at a stationary point, its corresponding network should interpolate a certain macroscopic data that consists of at most $n$ averaged points.
Motivated by this result, we propose a novel training scheme that not only accelerates the training but also reduce computational costs drastically.

\textcolor{red}{Thinking a way to extend this idea to a general deep ReLU network. I}
